Significance of Anatomical Constraints in Virtual Try-On

The system of Virtual Try-ON (VTON) allows a user to try a product virtually. In general, a VTON system takes a clothing source and a person's image to predict the try-on output of the person in the given clothing. Although existing methods perform well for simple poses, in case of bent or crossed arms posture or when there is a significant difference between the alignment of the source clothing and the pose of the target person, these methods fail by generating inaccurate clothing deformations. In the VTON methods that employ Thin Plate Spline (TPS) based clothing transformations, this mainly occurs for two reasons - (1)~the second-order smoothness constraint of TPS that restricts the bending of the object plane. (2)~Overlaps among different clothing parts (e.g., sleeves and torso) can not be modeled by a single TPS transformation, as it assumes the clothing as a single planar object; therefore, disregards the independence of movement of different clothing parts. To this end, we make two major contributions. Concerning the bending limitations of TPS, we propose a human AnaTomy-Aware Geometric (ATAG) transformation. Regarding the overlap issue, we propose a part-based warping approach that divides the clothing into independently warpable parts to warp them separately and later combine them. Extensive analysis shows the efficacy of this approach.

==> key_contribution_relevancetoTETCI.tex <==
Our proposed virtual try-on method performs significantly better for complex human postures achieving a 4.5\% improvement over SOTA. Our key contributions are
1. We propose a self-supervised model-to-person VTON solution that shows significant performance improvement over the previous methods, especially for complex human arm poses.
2. We propose a part-based solution approach by warping the independently movable parts separately.
3. We propose a hand-crafted feature-based warping method (ATAG transform) that is consistent with the geometry of the human arm.
4. Our proposed Mask Prediction Network (MPN) aids in identifying the occluded regions of the target clothing in the source and thereby guides the proposed Image Synthesizer Network (ISN) to predict lost clothing details in those regions.

This journal focuses on emerging topics and virtual try-on is a very promising and impactful technology in current times due to the immense impact it has on fashion industries related to e-commerce. 

The objective of Virtual Try-On is to synthesize an image of a person wearing a given clothing. Our method differs from the previous methods in terms of its approach to transforming the source clothing into its target form, which significantly improves the performance in the case of complex human postures. Quantitatively, we accomplish the best FID (Frechet Inception Distance) value of 15.74 achieving a 4.5\% improvement over SOTA. 

Specifically, our contributions can be summarized as the following, 
1. We propose a self-supervised model-to-person VTON solution that shows significant performance improvement over the previous methods, especially for complex human arm poses (see Fig.~\ref{fig: demo}).
2. We propose a part-based solution approach that addresses the overlap issues by warping the independently movable parts separately.
3. We discuss the limitations of the TPS transform in the current problem context and propose a hand-crafted feature-based warping method (ATAG transform) that is consistent with the geometry of the human arm. 
4. Our proposed Mask Prediction Network (MPN) aids in identifying the occluded regions of the target clothing in the source and thereby guides the proposed Image Synthesizer Network (ISN) to predict lost clothing details in those regions.

This journal focuses on emerging topics and virtual try-on is a very popular and impactful technology in current times due to the immense amount of revenue coming from fashion industries related to e-commerce. Hence, I believe this topic well relates to the goal of this journal.




The system of Virtual Try-ON (VTON) allows a user to try a product virtually. In general, a VTON system takes a clothing source and a person's image to predict the try-on output of the person in the given clothing. Although existing methods perform well for simple poses, in case of bent or crossed arms posture or when there is a significant difference between the alignment of the source clothing and the pose of the target person, these methods fail by generating inaccurate clothing deformations. In the VTON methods that employ Thin Plate Spline (TPS) based clothing transformations, this mainly occurs for two reasons - (1)~the second-order smoothness constraint of TPS that restricts the bending of the object plane. (2)~Overlaps among different clothing parts (e.g., sleeves and torso) can not be modelled by a single TPS transformation, as it assumes the clothing as a single planar object; therefore, disregards the independence of movement of different clothing parts. To this end, we make two major contributions. Concerning the bending limitations of TPS, we propose a human AnaTomy-Aware Geometric (ATAG) transformation.  Regarding the overlap issue, we propose a part-based warping approach that divides the clothing into independently warp-able parts to warp them separately and later combine them. Extensive analysis shows the efficacy of this approach which accomplishes the best FID value of 15.74 achieving a 4.5\% improvement over SOTA.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
